Byzantine Multiple Access Channels -- Part II: Communication With Adversary Identification

We introduce the problem of determining the identity of a byzantine user (internal adversary) in a communication system. We consider a two-user discrete memoryless multiple access channel where either user may deviate from the prescribed behaviour. Since small deviations may be indistinguishable from the effects of channel noise, it might be overly restrictive to attempt to detect all deviations. When neither user deviates, correct decoding is required. When one user deviates, the decoder must either output a pair of messages of which the message of the non-deviating user is correct or identify the deviating user. The users and the receiver do not share any randomness. The results include a characterization of the set of channels where communication is feasible, and an inner and outer bound on the capacity region. We also show that whenever the rate region has non-empty interior, the capacity region is same as the capacity region under randomized encoding, where each user shares independent randomness with the receiver. We also give an outer bound for this randomized coding capacity region.

==> converse.tex <==
%!TeX root=paper.tex
We start with a proof of the converse.
\begin{lemma}\label{thm:converse}
 If a channel is \one-spoofable (resp. \two-\spoofable), then  for any $(N_{\one}, N_{\two}, n)$ strongly authenticating code with $N_{\one}\geq 2$ (resp. $N_{\two}\geq 2$), the probability of error is at least $1/12$.  
 \end{lemma}
\begin{proof}
The proof uses ideas from proof of \cite[Lemma 1, page 187]{CsiszarN88}. Suppose the channel satisfies \eqref{eq:spoof1}. A similar analysis can be done when channel satisfies \eqref{eq:spoof2}. Let $Q_{Y|\tilde{X}, \tilde{Y}}$ and $Q_{X|\tilde{X},X'}$ be attacks satisfying \eqref{eq:spoof1}. For any given $(N_{\one}, N_{\two},n) $ code $(f_{\one},f_{\two}, \phi)$, let $i, j\in \cM_{\one}$ be distinct. For $i \in \cM_{\one}$, let $\vecx_{i} = f_{\one}(i)$. Similarly, for $k\in \cM_{\two}$, let $\vecy_{k}$ denote $f_{\two}(k)$. Consider the following situations.
\begin{itemize}
	\item User \one sends $\vecx_{i}$. User \two is adversarial and its input to the channel is produced by passing $(\vecx_{j}, \vecy_k)$ through the n-fold product channel $Q_{Y|\tilde{X}, \tilde{Y}}$. For $\vecz\in \cZ^n$, the output distribution $\bbP(\vecz)$ (denoted by $P_{i,j,k}(\vecz)$) is given by 
	\begin{align}\label{eq:dist1}
	P_{i,j,k}(\vecz) = \prod_{t=1}^n\sum_{y\in\cY}Q_{Y|\tilde{X}, \tilde{Y}}(y|\vecx_{j}(t),\vecy_{k}(t))W_{Z|X,Y}(\vecz(t)|\vecx_{i}(t),y).
	\end{align}
	
	
	\item User \two sends  $\vecy_k$. User \one is adversarial and its input $\vecX_{i,j}$ to the channel is produced by passing $(\vecx_{i}, \vecx_{j})$ through the n-fold product channel $Q_{X|\tilde{X}, X'}$.  For $\vecz\in \cZ^n$, the output distribution $\bbP(\vecz)$ (denoted by $Q_{i,j,k}(\vecz)$) is given by 
\begin{align}\label{eq:dist2}
	Q_{i,j,k}(\vecz) = \prod_{t=1}^n\sum_{x\in\cX}Q_{X|\tilde{X}, X'}(x|\vecx_{i}(t),\vecx_{j}(t))W_{Z|X,Y}(\vecz(t)|x,\vecy_{k}(t)).
	\end{align}
\end{itemize}
By \eqref{eq:spoof1}, we see that for all $i,j\in \cM_{\one}, k\in \cM_{\two}$ and $\vecz\in \cZ^n$, $P_{i,j,k}(\vecz)=P_{j,i,k}(\vecz)=Q_{i,j,k}(\vecz)$. From \eqref{eq:mal2} and \eqref{eq:dist1}, we see that
\begin{align*}
P_{e,\maltwo}&\geq \frac{1}{N^2_{\one}\times N_{\two}}\sum_{i,j\in\cM_{\one}}\sum_{k\in \cM_{\two}}\sum_{\vecz:\phi_{\one}(\vecz)\notin\{i,\two\}}P_{i,j,k}(\vecz)
\end{align*} and 
\begin{align*}
P_{e,\maltwo}&\geq \frac{1}{N^2_{\one}\times N_{\two}}\sum_{i,j\in\cM_{\one}}\sum_{k\in \cM_{\two}}\sum_{\vecz:\phi_{\one}(\vecz)\notin\{j,\two\}}P_{j,i,k}(\vecz).
\end{align*} Using \eqref{eq:mal1} and \eqref{eq:dist2}, we obtain
\begin{align*}
P_{e,\malone}&\geq \frac{1}{N^2_{\one}\times N_{\two}}\sum_{i,j\in\cM_{\one}}\sum_{k\in \cM_{\two}}\sum_{\vecz:\phi_{\two}(\vecz)\notin\{k,\one\}}Q_{i,j,k}(\vecz).
\end{align*}
\noindent Thus,
\begin{align*}
3&P_{e}(f_{\one},f_{\two},\phi)\geq P_{e,\maltwo}+P_{e,\maltwo}+P_{e,\malone}\\
&\geq \frac{1}{N^2_{\one}\times N_{\two}}\sum_{i,j\in\cM_{\one}}\sum_{k\in \cM_{\two}}\inp{\sum_{\vecz:\phi_{\one}(\vecz)\notin\{i,\two\}}P_{i,j,k}(\vecz) + \sum_{\vecz:\phi_{\one}(\vecz)\notin\{j,\two\}}P_{j,i,k}(\vecz) +\sum_{\vecz:\phi_{\two}(\vecz)\notin\{k,\one\}}Q_{i,j,k}(\vecz) }\\
&\stackrel{\text{(a)}}{=}\frac{1}{N^2_{\one}\times N_{\two}}\sum_{i,j\in\cM_{\one}}\sum_{k\in \cM_{\two}}\inp{\sum_{\vecz:\phi_{\one}(\vecz)\notin\{i,\two\}}P_{i,j,k}(\vecz) + \sum_{\vecz:\phi_{\one}(\vecz)\notin\{j,\two\}}P_{i,j,k}(\vecz) +\sum_{\vecz:\phi_{\two}(\vecz)\notin\{k,\one\}}P_{i,j,k}(\vecz) }\\
&\geq\frac{1}{N^2_{\one}\times N_{\two}}\sum_{i,j\in\cM_{\one}, i\neq j}\sum_{k\in \cM_{\two}}\inp{\sum_{\vecz\in\cZ^n}P_{i,j,k}(\vecz)}\\
&=\frac{N_{\one}(N_{\one}-1)N_{\two}}{2N^2_{\one}\times N_{\two}}\\
& = \frac{N_{\one}-1}{2N_{\one}}\\
&\geq \frac{1}{4}
\end{align*}
where (a) follows by noting that $P_{i,j,k}(\vecz)=P_{j,i,k}(\vecz)=Q_{i,j,k}(\vecz)$. Thus, for any given code $(f_{\one}, f_{\two}, \phi)$, for a spoofable channel $P_e(f_{\one},f_{\two}, \phi)\geq \frac{1}{12}$.
A similar analysis follows when the channel is \two-\spoofable.
\end{proof}


==> outerbound_proof.tex <==
%!TeX root=paper.tex
\section{Proof of Theorem~\ref{thm:outer_bd}}\label{sec:outer_bd_proof}
Consider an $(N_{\one}, N_{\two}, n)$ adversary identifying code $(F^{(n)}_{\one},F^{(n)}_{\two}, \Phi^{(n)})$ (with potential shared randomness between the encoder and the decoder) such that $P_{e}(F^{(n)}_{\one},F^{(n)}_{\two}, \Phi^{(n)}) \leq \epsilon(n)$ where $\epsilon(n)\rightarrow 0$ as $n\rightarrow 0$.
For for all $i\in [1:n]$, let $(Q^i_{X'|X}, Q^i_{Y'|Y})$ be an arbitrary sequence of pairs of channel distributions satisfying \eqref{eq:outer_bound}. Define $\tilde{W}_{i}$ as 
\begin{align*}
\tilde{W}_{i}(z|x,y) \defineqq \sum_{x'}Q^{i}_{X'|X}(x'|x)W(z|x',y) = \sum_{y'}Q^{i}_{Y'|Y}(y'|y)W(z|x,y') 
\end{align*}
for all $x,y,z$. Let $Q^{(n)}_{X'|X}\defineqq \prod_{i=1}^{n}Q^{i}_{X'|X}$, $Q^{(n)}_{Y'|Y}\defineqq \prod_{i=1}^{n}Q^{i}_{Y'|Y}$ and $\tilde{W}^{(n)} = \prod_{i=1}^{n}\tilde{W}_{i}$.

Then, 
\begin{align*}
P_{e, \malone} \geq \frac{1}{N_{\one}\cdot N_{\two}}\sum_{\mo, \mt}\sum_{\vecx}Q^{(n)}_{X'|X}(\vecx|F^{(n)}_{\one}(\mo))W^n\inp{\inb{\vecz:\Phi^{(n)}(\vecz) = \twob}\Big|\vecx,F_{\two}^{(n)}(\mt)}
\end{align*} and


\begin{align*}
P_{e, \maltwo} \geq \frac{1}{N_{\one}\cdot N_{\two}}\sum_{\mo, \mt}\sum_{\vecy}Q^{(n)}_{Y'|Y}(\vecx|F^{(n)}_{\two}(\mt))W^n\inp{\inb{\vecz:\Phi^{(n)}(\vecz) = \oneb}\Big|F_{\one}^{(n)}(\mo), \vecy}.
\end{align*}
Using these two equations, we get
\begin{align*}
2\epsilon(n)&\geq P_{e, \malone} + P_{e, \maltwo} \geq \frac{1}{N_{\one}\cdot N_{\two}}\sum_{\mo, \mt}\Big(\sum_{\vecx}Q^{(n)}_{X'|X}(\vecx|F^{(n)}_{\one}(\mo))W^n\inp{\inb{\vecz:\Phi^{(n)}(\vecz) = \twob}\Big|\vecx,F_{\two}^{(n)}(\mt)}\\
&\qquad+ \sum_{\vecy}Q^{(n)}_{Y'|Y}(\vecy|F^{(n)}_{\two}(\mt))W^n\inp{\inb{\vecz:\Phi^{(n)}(\vecz) = \oneb}\Big|F_{\one}^{(n)}(\mo), \vecy}\Big)\\
& = \frac{1}{N_{\one}\cdot N_{\two}}\sum_{\mo, \mt}\tilde{W}^{(n)}\inp{\inb{\vecz:\Phi^{(n)}(\vecz) \in \{\oneb, \twob\}}\Big|F^{(n)}_{\one}(\mo),F_{\two}^{(n)}(\mt)}.
\end{align*}
Thus, 
\begin{align*}
&\frac{1}{N_{\one}\cdot N_{\two}}\sum_{\mo, \mt}\tilde{W}^{(n)}\inp{\inb{\vecz:\Phi^{(n)}(\vecz) \neq (\mo, \mt)}|F^{(n)}_{\one}(\mo),F_{\two}^{(n)}(\mt)} \\
&= \frac{1}{N_{\one}\cdot N_{\two}}\sum_{\mo, \mt}\tilde{W}^{(n)}\inp{\inb{\vecz:\Phi^{(n)}(\vecz) \in \cM_{\one}\times\cM_{\two}\setminus\{(\mo, \mt)\}}|F^{(n)}_{\one}(\mo),F_{\two}^{(n)}(\mt)}\\
&\qquad + \frac{1}{N_{\one}\cdot N_{\two}}\sum_{\mo, \mt}\tilde{W}^{(n)}\inp{\inb{\vecz:\Phi^{(n)}(\vecz) \in \{\oneb, \twob\}}\Big|F^{(n)}_{\one}(\mo),F_{\two}^{(n)}(\mt)}\\
&\leq \epsilon(n) + 2\epsilon(n)\\
&= 3\epsilon(n).
\end{align*}
Recall that every pair $(Q_{X'|X}, Q_{Y'|Y})$ satisfying \eqref{eq:outer_bound} corresponds to an element in $\tilde{\cW}_W$ which is a convex set (see the discussion in Section~\ref{sec:outer_bd}). Thus, any adversary identifying code for the MAC $W$ with probability of error $\epsilon(n)$ is also a communication code for the AV-MAC $\tilde{\cW}_{W}$ with probability of error at most $3\epsilon(n)$. So, capacity region of $W$ is outer bounded by the capacity region of the AV-MAC $\tilde{\cW}_{W}$. 

The capacity of an AV-MAC only depends on its convex hull \cite{Jahn81}. So, capacity of $\tilde{\cW}_{W}$ is same as capacity of another AV-MAC $\cW_{W}$ which consists of vertices of the convex polytope $\tilde{\cW}_{W}\subseteq \bbR^{|\cX|\times|\cY|\times|\cZ|}$.
The elements in the set $\tilde{\cW}_{W}$ are parameterized by $(Q_{X'|X}, Q_{Y'|Y})$ pairs. It consists of the vertices of the polytope formed using constraints in \eqref{eq:outer_bound} and constraints of the form: (1) $\sum_{x'}P_{X'|X}(x'|x) = 1$ for all $x$, and (2) $P_{X'|X}(x'|x)\geq 0$. There are similar constraints for $P_{Y'|Y}$. Note that there are $|X|^2 + |Y|^2$ inequality constraints. Every point in the resulting polytope satisfies all the equality constraints. We will get faces, edges, vertices etc. depending on the number of additional inequality constraints satisfied at that point. Thus, number of vertices $\leq 2^{|X|^2 + |Y|^2}$.


